Discrete Diffusion Models for Language Generation

Diffusion models have emerged as a powerful class of generative models, achieving state-of-the-art results in continuous data domains such as image and video generation. Their core mechanism involves a forward diffusion process that gradually transforms structured data into a Gaussian-like distribution, followed by a learned reverse process to reconstruct the data. While successful in continuous modalities, applying this framework to discrete data-particularly natural language-remains challenging due to token dependency complexities and the lack of a defined generation order.This thesis investigates the feasibility and performance of discrete diffusion models for natural language generation. Specifically, we evaluate the Discrete Denoising Diffusion Probabilistic Model (D3PM) and compare it with traditional autoregressive (AR) language models. To assess generative performance, we use Bits Per Token (BPT), Negative Log-Likelihood (NLL), Perplexity (PPL), and Batch Processing Speed. Results show the best-performing D3PM model achieves a BPT of 5.72, with a mean of 8.05. The AR model outperforms in compression with a lower mean BPT of 4.59, but D3PM achieves higher processing speed, reaching up to 3.97 batches per sec., indicating potential for parallel generation.All evaluations were conducted under consistent conditions-generating 100,000 tokens per model with a fixed batch size of four-for fair comparison. This research presents a detailed analysis of diffusion-based vs. autoregressive models, highlighting trade-offs in generative quality and efficiency. Findings emphasize both the promise and limitations of diffusion models for discrete data, supporting future work in non-autoregressive language generation.

==> abstract.tex <==
%%% Abstract.tex --- 
%% 
%% Filename: Abstract.tex
%% Description: 
%% Author: Ola Leifler
%% Maintainer: 
%% Created: Thu Oct 14 13:34:11 2010 (CEST)
%% Version: $Id$
%% Version: 
%% Last-Updated: Fri Jan 14 08:48:50 2022 (+0100)
%%           By: Ola
%%     Update #: 6
%% URL: 
%% Keywords: 
%% Compatibility: 
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Commentary: 
%% 
%% 
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Change log:
%% 
%% 
%% RCS $Log$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Code:

Diffusion models have emerged as a powerful class of generative models, achieving state-of-the-art performance in continuous data domains such as image synthesis and video generation. Their core mechanism involves a forward diffusion process that gradually transforms structured data into a Gaussian-like distribution, followed by a learned reverse diffusion process that reconstructs the data. While this framework has proven effective for continuous modalities, its application to discrete data—particularly natural language—remains a challenging and active area of research. \cite{austin2021structured} Key obstacles include the complexity of modeling discrete token dependencies and the lack of a naturally defined generation order.

This thesis investigates the feasibility and performance of discrete diffusion models in the context of natural language generation. In particular, we examine the Discrete Denoising Diffusion Probabilistic Model (D3PM)\ref{sec:d3pm} and compare its performance against traditional autoregressive (AR)\ref{sec:ar} language models. To evaluate and compare the generative capacity of both models, we utilize common metrics such as Bits Per Token (BPT)\ref{sec:bpt}, Negative Log-Likelihood (NLL)\ref{sec:nll}, Perplexity (PPL)\ref{sec:ppl}, and Batch Processing Speed.

Experimental results\ref{cha:results} show that the best-performing D3PM model achieves a BPT of 5.72, with a mean value of 8.05 across runs. In contrast, the AR model demonstrates a lower mean BPT of 4.59, indicating better compression and generative efficiency. However, D3PM models achieve higher batch processing speeds, with a maximum of 3.97 batches per second, highlighting their potential for parallel generation.

All evaluations were conducted under consistent conditions—generating 100,000 tokens per model with a fixed batch size of four—to ensure fairness and comparability. This research contributes a detailed comparative analysis of diffusion-based and autoregressive models, offering insights into their respective trade-offs. Ultimately, the findings underscore both the promise and the current limitations of applying diffusion models to discrete sequence modeling, and provide a foundation for future exploration in non-autoregressive language generation frameworks.The source code used in this research is available at the following GitHub repository: \url{https://github.com/AshenWELI/Discrete-Diffusion-Models-for-Language-Genaration}.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Abstract.tex ends here


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "demothesis"
%%% End: 


==> acknowledgments.tex <==
%%% Acknowledgments.tex<2> --- 
%% 
%% Filename: Acknowledgments.tex<2>
%% Description: 
%% Author: Ola Leifler
%% Maintainer: 
%% Created: Wed Nov 10 09:45:11 2010 (CET)
%% Version: $Id$
%% Version: 
%% Last-Updated: Tue Jun 21 13:28:03 2016 (+0200)
%%           By: Ola Leifler
%%     Update #: 6
%% URL: 
%% Keywords: 
%% Compatibility: 
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Commentary: 
%% 
%% 
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Change log:
%% 
%% 
%% RCS $Log$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Code:

\swedishenglish{\chapter*{Författarens tack}}{\chapter*{Acknowledgments}}

First of all, I would like to thank my supervisor, Dr. Dong Qian, for guiding me to understand the deep knowledge behind this thesis. He always taught me how to understand the question — no matter how crazy it was. Our discussions were always exciting, and they helped clear my mind and opened my eyes to new insights. He constantly encouraged me to succeed. Thank you for everything you have done.

Then, I would like to thank Prof. Anders Eklund for guiding me in successfully dealing with high-performance computing. At first, it was a bit tricky for me, but I got valuable advice from him. I never expected that much help, and as much as I could, I discussed and shared the status of my model with him.

Gratitude also extends to my examiner, Prof. Zheng Zhao, and my opponent, Greeshma Jeev Koothuparambil, for pointing out the flaws in my story, correcting the mistakes, and helping to edit it in a way that the reader can follow the theory meaningfully.

Secondly, I want to remember my home country supervisor, Dr. Rushan Abeygunawardana, for encouraging my academics. I also want to thank my friends who helped me understand the unknown parts: Tharuka Mannapperuma and Tharuka Shayaman.

Finally, I want to thank my backbone — my mom, Anoma Karunasekara, and dad, Amarabandu Weligalle — for helping and encouraging me through everything, and for supporting me in this unknown, cold country. In the end, my little sister, Manushi Weligalle, always helped relax my mind and took it off the thesis, even during tough times. I always remember my family and am deeply thankful for helping me complete this.

\vspace{1em}
\begin{center}
\textit{Thank you all who helped me to complete this!}
\end{center}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Acknowledgments.tex<2> ends here

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "demothesis"
%%% End: 


==> pdftopdfa <==
#! /usr/bin/env bash
filenames=${@%.pdf}
#### Use sRGB for now, proper color profile handling likely first in latex-3
#  -sColorConversionStrategy=UseDeviceIndependentColor 
for filename in ${filenames[@]}; do
  echo Converting ${filename}.pdf
  gs -dPDFA -dBATCH -dNOPAUSE              \
    -sColorConversionStrategy=RGB          \
    -sDEVICE=pdfwrite                      \
    -dPDFACompatibilityPolicy=3            \
    -sOutputFile=${filename}_pdfa_rgb.pdf  \
     ${filename}.pdf
  gs -dPDFA -dBATCH -dNOPAUSE              \
    -sColorConversionStrategy=CMYK         \
    -sDEVICE=pdfwrite                      \
    -dPDFACompatibilityPolicy=3            \
    -sOutputFile=${filename}_pdfa_cmyk.pdf \
     ${filename}.pdf
done


==> sammanfattning.tex <==
%%% sammanfattning.tex --- 
%% 
%% Filename: sammanfattning.tex
%% Description: 
%% Author: Ola Leifler
%% Maintainer: 
%% Created: Thu Oct 14 13:34:11 2010 (CEST)
%% Version: $Id$
%% Version: 
%% Last-Updated: Thu Apr 13 11:36:41 2017 (+0200)
%%           By: Ola Leifler
%%     Update #: 8
%% URL: 
%% Keywords: 
%% Compatibility: 
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Commentary: 
%% 
%%  Populärvetenskaplig sammanfattning av arbetet på svenska
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Change log:
%% 
%% 
%% RCS $Log$
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% 
%%% Code:

\texttt{Populärvetenskaplig sammanfattning på svenska i sammanfattning.tex}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% sammanfattning.tex ends here


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "demothesis"
%%% End: 

